Towards Reliable LLM-Driven Fuzz Testing: Vision and Road Ahead

Fuzz testing is a crucial component of software security assessment, yet its effectiveness heavily relies on valid fuzz drivers and diverse seed inputs. Recent advancements in Large Language Models (LLMs) offer transformative potential for automating fuzz testing (LLM4Fuzz), particularly in generating drivers and seeds. However, current LLM4Fuzz solutions face critical reliability challenges, including low driver validity rates and seed quality trade-offs, hindering their practical adoption. This paper aims to examine the reliability bottlenecks of LLM-driven fuzzing and explores potential research directions to address these limitations. It begins with an overview of the current development of LLM4SE and emphasizes the necessity for developing reliable LLM4Fuzz solutions. Following this, the paper envisions a vision where reliable LLM4Fuzz transforms the landscape of software testing and security for industry, software development practitioners, and economic accessibility. It then outlines a road ahead for future research, identifying key challenges and offering specific suggestions for the researchers to consider. This work strives to spark innovation in the field, positioning reliable LLM4Fuzz as a fundamental component of modern software testing.

==> RQ1.tex <==
\section{RQ1: How LLMs are Utilized?}
In this section, we illustrate which LLMs and strategies are utilized in the fuzz driver and seed generation tasks.

\subsection{Models Utilized in LLM-based Fuzzing}
Several fuzzing approaches employ multiple LLMs for different stages of their workflow, such as Fuzz4all which utilizes GPT-4 as a distillation LLM for autoprompting and StarCoder as a generation LLM for producing fuzzing inputs. 
The GPT series models from OpenAI have been widely adopted in LLM-based fuzzing studies, with GPT-4 being utilized in 43.8\% (7/16) studies, while GPT-3.5 and GPT-3 have been adopted in 37.5\% (6/16) and 12.5\% (2/16) respectively. Beyond the GPT family, DeepSeek-V2, also as a general language model has been used in Fuzz4all.
Open-source code generation models have also played a crucial role, with StarCoder and Incoder each being employed in 12.5\% (2/16) studies, while models like Codellama and Wizardcoder have shown promise in specific implementations. 
Additionally, some researchers have explored code understanding models such as CodeBERT and UniXcoder, which are particularly adept at tasks requiring deep code comprehension due to their pre-training in both programming languages and natural language.

\subsection{Prompt Strategies}
The prompt strategies employed across these studies reveal a sophisticated approach to leveraging LLMs for fuzzing tasks. 
Chain-of-Thought (CoT) prompting has emerged as a fundamental technique, enabling structured reasoning for complex tasks such as crash analysis and bug prediction. This approach is often complemented by step-by-step prompting, which helps decompose complex fuzzing tasks into manageable sequences. 
Knowledge enhancement strategies have proven crucial, with several studies incorporating code knowledge graphs, API documentation, and contextual information into their prompts. 
The implementation of few-shot learning techniques has been particularly effective, where carefully selected examples guide the models toward generating more accurate and relevant outputs. Quality assurance has been addressed through various mechanisms, including self-consistency checks and iterative refinement processes. 
Temperature parameter tuning has been strategically employed, with studies using lower values (0) for deterministic outputs in critical tasks and higher values (0.7-0.9) when more creative generation is desired. 
The prompting strategies often vary based on the specific fuzzing task, with driver generation focusing on API understanding and usage patterns, while seed generation emphasizes mutation and exploration strategies. These approaches are frequently combined and adapted, with researchers carefully balancing the trade-offs between precision and creativity in their prompt designs.
